VF-NeRF: Viewshed Fields for Rigid NeRF Registration

3D scene registration is a fundamental problem in computer vision that seeks the best 6-DoF alignment between two scenes. This problem was extensively investigated in the case of point clouds and meshes, but there has been relatively limited work regarding Neural Radiance Fields (NeRF). In this paper, we consider the problem of rigid registration between two NeRFs when the position of the original cameras is not given. Our key novelty is the introduction of Viewshed Fields (VF), an implicit function that determines, for each 3D point, how likely it is to be viewed by the original cameras. We demonstrate how VF can help in the various stages of NeRF registration, with an extensive evaluation showing that VF-NeRF achieves SOTA results on various datasets with different capturing approaches such as LLFF and Objaverese.

==> Tables/LLFF_ablation.tex <==
% \begin{table}
\begin{wraptable}{R}{0.5\textwidth}
\centering
\vspace{0pt}
\begin{tabular}{lcc}

\toprule
\textbf{Model} &\textbf{$10^2 \cdot \Delta t \downarrow$} &\textbf{$\Delta R \downarrow$}\\
\midrule

No initialization 
&39.2993 &21.5474\\

No VF Masks
&1.7348 &1.3609\\

Single image
&9.4008 &8.9252\\

\textbf{Full method}
&\textbf{0.0151} &\textbf{0.0206}\\
 
\bottomrule

\end{tabular}

\caption{\textbf{Ablation study:} Rotation and translation RMS error comparison on LLFF dataset where each row represents an experiment with reduced abilities as stated. The results are the mean error over all the scenes in the LLFF dataset.
}
\label{Tab:LLFF_albation}
% \end{table} 
\end{wraptable}

==> Tables/noise_table.tex <==
% \begin{table}
\begin{wraptable}{R}{0.5\textwidth}
\centering
\vspace{0pt}
\begin{tabular}{lcc}

\toprule
\textbf{Noise} &\textbf{$10^2 \cdot \Delta t \downarrow$} &\textbf{$\Delta R \downarrow$}\\
\midrule

0\%  &
\textbf{0.0113} & 0.0108\\
1\% &
0.0114 & 0.0120\\
5\% &
0.0117 & \textbf{0.0106}\\
10\% &
0.0265 & 0.0140\\
20\% &
0.0149 & 0.0155\\

\bottomrule

\end{tabular}

\caption{\textbf{Noise Ablation study:} Rotation and translation RMS error comparison on Trex scene from LLFF dataset where each row represents an experiment with noised oriented points. specifically, we add a small random value proportionally to the scene size, for example 5\% represents noise values from a uniform distribution of [-5\%, 5\%] of the scene size. The results are the mean error over the tree overlap types.
}
\label{Tab:noise_ablation}
% \end{table} 
\end{wraptable}

==> Tables/objaverse_full_a.tex <==
\begin{table*}[!h]
   \caption{Quantitative results of registration on the Objaverse dataset - Part A. $\Delta \mathbf{R}$ denotes the relative rotation errors in degree, $\Delta \mathbf{t}$ denotes the relative translation errors multiplied by 1e2 with unknown scales. $\text{DReg}_{\text{df}}$ refers to DReg with density fields and DReg refers to DReg with surface field. FPFH + RANSAC uses point clouds generated by Viewshed Fields. VF-NeRF + PC Init refers to our algorithm after initializing with VF-based points clouds using FPFH + RANSAC. The results of FGR, REGTR and DReg are taken from ~\cite{chen2023dregnerf}.} 
  \centering
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Part 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \resizebox{0.98\textwidth}{!}{
    % \begin{tabular}{c | c c c c c c c c c c c c c c}
    % \begin{tabular}{c | l l l l l l l l l l l l l l}
    \begin{tabular}{c | l r r r r r r r r r r r r}
      \toprule

        &  & 
        \multicolumn{1}{l}{\textbf{Food 5648}} & \multicolumn{1}{l}{\textbf{Chair 4b05}} &  
        \multicolumn{1}{l}{\textbf{Chair 4659}} & \multicolumn{1}{l}{\textbf{Chair 3f2d}} &
        \multicolumn{1}{l}{\textbf{Cone 37b5}} & \multicolumn{1}{l}{\textbf{Figurine 260d}} & 
        \multicolumn{1}{l}{\textbf{Figurine 0a5b}} & \multicolumn{1}{l}{\textbf{Figurine 09f0}} & \multicolumn{1}{l}{\textbf{Banana 3a07}} & \multicolumn{1}{l}{\textbf{Banana 2373}} & \multicolumn{1}{l}{\textbf{Banana 0a07}}
      \\
      
      \midrule

      \multirow{4}{*}{$\Delta \mathbf{R}$} 
      & FGR~\cite{zhou2016fast} & 178.34 &  50.50 &  28.54 &  81.31 & 104.52 &  89.13 &  26.35 & 138.00 &  12.17 &   6.92 &   2.86
                                           \\
      & REGTR~\cite{yew2022regtr} & 169.07 & 150.38 &  92.80 &  98.67 &  62.50 & 111.80 & 106.12 & 176.48 & 136.02 & 178.36 & 173.96
                                           \\
      & $\text{DReg}_{\text{df}}$~\cite{chen2023dregnerf} & 77.48 & 160.13 & 157.21 & 22.91 & 108.09 & 121.32 & 10.53 & 95.89 & 95.43 & 3.49 & 6.96  \\
      % performance improved after tuning.
      & DReg~\cite{chen2023dregnerf} & 6.01 &  6.53 & 17.74 & 18.88 & \textbf{18.79} & 2.11 & 7.62 & 8.25 & 15.55 & 10.95 & 1.36
                         \\
      & FPFH~\cite{5152473} + RANSAC~\cite{10.1145/358669.358692} & 3.69 & 3.11 & 1.91 & 4.06 & 54.52 & 4.31 & 4.27 & 9.80 & 2.06 & 1.69 & 1.74
                         \\
      & VF-NeRF + PC Init.    & \textbf{0.03} & \textbf{0.03} & \textbf{0.03} & \textbf{0.80} & 49.05 & \textbf{0.84} & \textbf{0.60} & \textbf{0.92} & \textbf{0.03} & \textbf{1.28} & \textbf{0.03}
      \\


      \hline
      
      \multirow{4}{*}{$\Delta \mathbf{t}$} 
      & FGR~\cite{zhou2016fast} & 17.44 &  \textbf{2.27} &  7.10 &  8.65 &  30.49 & 19.25 & 10.93 & 35.22 &  8.50 & 1.53  &  1.36
                                           \\
      & REGTR~\cite{yew2022regtr} & 30.72 & 15.41 & 24.97 & 60.53 &  84.20 & 62.07 & 35.48 & 42.10 & 10.75 & 50.40 & 13.17
                                           \\
      & $\text{DReg}_{\text{df}}$~\cite{chen2023dregnerf} & 15.52 & 7.32 & 11.72 & 2.29 & 21.70 & 33.61 & 1.95 & 21.40 & 13.14 & 4.28 & 0.50 \\
      & DReg~\cite{chen2023dregnerf} &  1.78 & 4.13 & 8.74 & 5.07 & \textbf{3.06} & 3.54 & 10.68 & 3.18 & 0.46  & 1.00 & 1.22  
                         \\
      & FPFH~\cite{5152473} + RANSAC~\cite{10.1145/358669.358692} & 0.67 & \textbf{0.42} & 3.41 & \textbf{0.45} & 23.98 & 2.82 & 0.55 & 3.16 & 0.50 & \textbf{0.13} & 3.01
                         \\
      & VF-NeRF + PC Init. & \textbf{0.16} & 2.43 & \textbf{0.05} & 1.33 & 23.73 & \textbf{0.26} & \textbf{0.005} & \textbf{0.16} & \textbf{0.27} & 0.15 & \textbf{0.44}
      \\

      \bottomrule
    \end{tabular}
  }
  
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Part 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \resizebox{0.98\textwidth}{!}{
    % \begin{tabular}{c | c c c c c c c c c c c c c}
    % \begin{tabular}{c | l l l l l l l l l l l l l l}
    \begin{tabular}{c | l r r r r r r r r r r r r}
      \toprule

        &  & 
      \multicolumn{1}{l}{\textbf{Fireplug 06d5}} & \multicolumn{1}{l}{\textbf{Fireplug 0063}} & \multicolumn{1}{l}{\textbf{Fireplug 0152}} & \multicolumn{1}{l}{\textbf{Shoe 18c3}} &
      \multicolumn{1}{l}{\textbf{Shoe 1627}} & \multicolumn{1}{l}{\textbf{Shoe 0bf9}} &
      \multicolumn{1}{l}{\textbf{Shoe 022c}} & \multicolumn{1}{l}{\textbf{Teddy 1b47}} &
      \multicolumn{1}{l}{\textbf{Elephant 183a}} & \multicolumn{1}{l}{\textbf{Elephant 1608}} & \multicolumn{1}{l}{\textbf{Elephant 1a39}}
      \\
      
      \midrule

      \multirow{4}{*}{$\Delta \mathbf{R}$} 
      & FGR~\cite{zhou2016fast} & 6.19 & 20.32 &  7.50 & 10.23 & 178.14 & 71.55 & 50.28 & 8.05 & 7.65 &  21.37 & 30.97
                                           \\
      & REGTR~\cite{yew2022regtr}  & 156.92 & 99.60 & 4.04 & 2.55 & 175.21 &  97.92 &  154.91 & 149.17 & 177.15 & 172.28 & 102.62
                                            \\
      & $\text{DReg}_{\text{df}}$~\cite{chen2023dregnerf} & 156.17 & 45.76 & 12.34 & 14.69 & 131.66 & 158.66 & 6.84 & 6.32 & 6.97 & 3.92 & 126.94
                                  \\
      & DReg~\cite{chen2023dregnerf} & 7.96 & 17.43 &  4.86 & 6.06 & \textbf{12.95} & \textbf{6.48} & 2.93 & 11.44 & 8.00 & 11.13 & 13.84
                         \\
      & FPFH~\cite{5152473} + RANSAC~\cite{10.1145/358669.358692} &      5.65 & 2.06 & 1.53 & 2.07 & 14.38 & 6.44 & 2.96 & 7.14 & 1.23 & 8.30 & 1.28                   
      \\
      & VF-NeRF + PC Init. & \textbf{0.36} & \textbf{0.03} & \textbf{1.11} & \textbf{1.06} & \textbf{1.00} & \textbf{5.38} & \textbf{0.03} & \textbf{6.07} & \textbf{1.09} & \textbf{3.25} & \textbf{0.71}
      \\
      \hline
      
      \multirow{4}{*}{$\Delta \mathbf{t}$} 
      & FGR~\cite{zhou2016fast} & 5.83 &  0.83 &  1.17 &  \textbf{0.04} & 4.99 & 8.82 &  35.47 &  1.11 & 4.51 & 14.08 & 11.03
                                           \\
      & REGTR~\cite{yew2022regtr} & 68.71 & 38.74 & 2.13 & 3.53 & 43.40 & 61.37 & 102.00 & 42.84 & 52.26 & 66.15 & 34.54
                                           \\
      & $\text{DReg}_{\text{df}}$~\cite{chen2023dregnerf} & 10.54 & 5.32 & 2.60 & 4.66 & 28.63 & 24.82 & 4.40 & 2.20 & 4.26 & \textbf{1.40} & 33.57  
                                  \\
      & DReg~\cite{chen2023dregnerf} & 1.58 & 5.08 & \textbf{0.96} & 2.08 & 12.80  & 1.81 & 0.65 & \textbf{1.06} & 8.97 & 6.17 & 7.80
                         \\
      & FPFH~\cite{5152473} + RANSAC~\cite{10.1145/358669.358692} & 0.47 & 0.17 & 2.98 & 1.33 & 7.40 & \textbf{1.08} & 2.05 & 6.54 & 0.30 & 3.88 & 0.86
                         \\
      & VF-NeRF + PC Init. & \textbf{0.006} & \textbf{0.023} & 2.60 & 0.24 & \textbf{0.13} & 4.56 & \textbf{0.19} & 5.90 & \textbf{0.17} & 2.57 & \textbf{0.76}
\\
      \bottomrule
    \end{tabular}
  }
 

 
   \label{table:full_objaverse_results}
  %  \vspace{-4mm}
\end{table*}


==> Tables/objaverse_full_b.tex <==
\begin{table*}[!h]
   \caption{Quantitative results of registration on the Objaverse dataset - Part B. $\Delta \mathbf{R}$ denotes the relative rotation errors in degree, $\Delta \mathbf{t}$ denotes the relative translation errors multiplied by 1e2 with unknown scales. $\text{DReg}_{\text{df}}$ refers to DReg with density fields and DReg refers to DReg with surface field. FPFH + RANSAC uses point clouds generated by Viewshed Fields. VF-NeRF + PC Init refers to our algorithm after initializing with VF-based points clouds using FPFH + RANSAC. The results of FGR, REGTR and DReg are taken from ~\cite{chen2023dregnerf}.} 
  \centering

   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Part 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   \resizebox{0.98\textwidth}{!}{
%      % \begin{tabular}{c | c c c c c c c c c c c c c c}
%      % \begin{tabular}{c | l l l l l l l l l l l l l l}
     \begin{tabular}{c | l r r r r r r r r r r r r}
       \toprule
 
         &  & 
         \multicolumn{1}{l}{\textbf{Piano 0e0d}} & \multicolumn{1}{l}{\textbf{Piano 0a6e}} &
         \multicolumn{1}{l}{\textbf{Truck 1431}} & \multicolumn{1}{l}{\textbf{Guitar 15b4}} & \multicolumn{1}{l}{\textbf{Guitar 14f8}} & \multicolumn{1}{l}{\textbf{Guitar 0ceb}} &
         \multicolumn{1}{l}{\textbf{Guitar 0aa0}} & \multicolumn{1}{l}{\textbf{Lantern 0231}} & \multicolumn{1}{l}{\textbf{Lamp 0230}} & \multicolumn{1}{l}{\textbf{Bench 0b05}} & \multicolumn{1}{l}{\textbf{Shield 22a7}} 
       \\
       
       \midrule
 
       \multirow{4}{*}{$\Delta \mathbf{R}$} 
       & FGR~\cite{zhou2016fast} & 23.09 & 77.63 & 7.46 & 7.80 & 5.25 & 13.07 & 39.94 & 130.36 & 17.44 & 19.51 & 170.27   
                                            \\
       & REGTR~\cite{yew2022regtr} & 30.54 & 117.90 & 178.49 & 5.18 & 29.47 & 103.84 & 5.95 & 139.32 & 160.45 & 122.12 & 157.38
                                            \\
       & $\text{DReg}_{\text{df}}$~\cite{chen2023dregnerf} & 160.71 & 168.79 & 117.07 & 11.43 & 164.87 & 177.62 & 7.96 & 7.76 & 173.09 & 179.16 & 178.00 \\
       % performance improved after tuning.
       & DReg~\cite{chen2023dregnerf} & 16.30 & 13.51 & 16.68 & 12.60 & 3.43 & \textbf{1.08} & 9.53 & 9.17 & 16.44 & 12.98 & 8.21
                          \\
      & FPFH~\cite{5152473} + RANSAC~\cite{10.1145/358669.358692} & \textbf{5.80} & 12.86 & 6.62 & 1.84 & 3.91 & 2.06 & 2.44 & 2.69 & 2.82 & 2.47 & \textbf{1.29}              
      \\
      & VF-NeRF + PC Init. & 6.89 & \textbf{6.37} & \textbf{0.03} & \textbf{1.34} & \textbf{1.98} & 1.16 & \textbf{1.54} & \textbf{0.83} & \textbf{0.03} & \textbf{0.03} & 3.68
      \\
       \hline
       
       \multirow{4}{*}{$\Delta \mathbf{t}$} 
       & FGR~\cite{zhou2016fast} & 7.43 & 14.50 & 5.95 & 2.86 & 3.46 & 1.83 & 8.42 & 9.06 & 0.69 & 12.52 & 15.57
                                            \\
       & REGTR~\cite{yew2022regtr} & 44.24 & 65.99 & 50.63 & 15.18 & 18.41 & 89.20 & 9.91 & 57.25 & 64.44 & 31.97 & 44.29
                                            \\
       & $\text{DReg}_{\text{df}}$~\cite{chen2023dregnerf} & 22.86 & 26.18 & 24.83 & 10.27 & 8.50 & 43.21 & 4.09 & 3.35 & 26.77 & 28.59 & 34.71 \\
       & DReg~\cite{chen2023dregnerf} & 4.80 & 12.54 & \textbf{0.04} & 5.72 & 5.03 & 3.01 & 1.20 & 3.29 & 1.31 & 1.68 & 11.33
                          \\
       & FPFH~\cite{5152473} + RANSAC~\cite{10.1145/358669.358692} & \textbf{3.74} & \textbf{3.14} & 4.27 & 2.15 & 1.05 & 1.47 & 1.16 & 2.43 & 0.91 & 5.43 & \textbf{3.07}
                         \\
      & VF-NeRF + PC Init. & 13.84 & 6.45 & 0.36 & \textbf{0.14} & \textbf{0.14} & \textbf{0.74} & \textbf{0.16} & \textbf{0.36} & \textbf{0.11} & \textbf{0.27} & 8.03
      \\
       \bottomrule
     \end{tabular}
   }
   
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Part 4 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   \resizebox{0.98\textwidth}{!}{
     % \begin{tabular}{c | c c c c c c c c c c c c c}
     % \begin{tabular}{c | l l l l l l l l l l l l l l}
     \begin{tabular}{c | l r r r r r r r r r r r r}
       \toprule
 
         &  & 
       \multicolumn{1}{l}{\textbf{Shield 1973}} & \multicolumn{1}{l}{\textbf{Shield 14a6}} &
       \multicolumn{1}{l}{\textbf{Shield 00ad}} & \multicolumn{1}{l}{\textbf{Controller 0866}} & \multicolumn{1}{l}{\textbf{Fighter Jet 16c6}} & \multicolumn{1}{l}{\textbf{Fighter Jet 089f}} & \multicolumn{1}{l}{\textbf{Fighter Jet 0000}} & \multicolumn{1}{l}{\textbf{Telephone 1a8c}} & \multicolumn{1}{l}{\textbf{Telephone 0354}} & \multicolumn{1}{l}{\textbf{Lampshade ab66}} & \multicolumn{1}{l}{\textbf{Skateboard 10c7}} 
       \\
       
       \midrule
 
       \multirow{4}{*}{$\Delta \mathbf{R}$} 
       & FGR~\cite{zhou2016fast} & 130.83 & 178.99 & 7.06 & 164.01 & 11.91 & 40.21 & 39.86 & 150.10 & 19.76 & 147.50 & 176.90
                                            \\
       & REGTR~\cite{yew2022regtr}  & 138.94 & 169.78 & 14.76 & 102.05 & 154.74 & 150.64 & 178.35 & 144.47 & 1.13 & 148.44 & 3.88
                                             \\
       & $\text{DReg}_{\text{df}}$~\cite{chen2023dregnerf} & 178.93 & \textbf{4.92} & 7.78 & 179.13 & 9.75 & 23.97 & 178.68 & 132.49 & 16.59 & 5.79 & 179.97 \\
       & DReg~\cite{chen2023dregnerf} & 12.94 & 12.26 & 2.29 & 4.03 & 6.88 & 10.53 & 6.46 & 15.60 & 9.01 & 5.67 & \textbf{1.92}
                          \\
       & FPFH~\cite{5152473} + RANSAC~\cite{10.1145/358669.358692} & 3.92 & 13.62 & \textbf{1.14} & 7.14 & 1.50 & 3.55 & \textbf{1.31} & 23.12 & 3.32 & 1.98 & 179.45
                         \\
      & VF-NeRF + PC Init. & \textbf{2.74} & 13.46 & 1.47 & \textbf{0.03} & \textbf{0.26} & \textbf{0.03} & 2.12 & \textbf{0.03} & \textbf{0.03} & \textbf{1.19} & 179.10
      \\
       \hline
       
       \multirow{4}{*}{$\Delta \mathbf{t}$} 
       & FGR~\cite{zhou2016fast} & 49.44 & 55.62 & \textbf{0.22} & 8.97 & 6.90 & 11.73 & 3.44 & 57.53 & 18.51 & 67.08 & 19.03
                                            \\
       & REGTR~\cite{yew2022regtr} & 72.01 & 48.56 & 6.57 & 65.87 & 52.97 & 82.10 & 28.79 & 51.09 & 0.91 & 54.45 & 5.14
                                            \\
       & $\text{DReg}_{\text{df}}$~\cite{chen2023dregnerf} & 59.08 & \textbf{0.66} & 1.58 & 23.68 & 2.64 & 13.98 & 19.28 & 63.76 & 15.65 & 4.81 & 12.20 \\
       & DReg~\cite{chen2023dregnerf} & 2.79 & 4.38 & 1.26 & \textbf{0.99} & 2.53 & 7.55 & 2.09 & 1.28 & 3.57 & \textbf{0.81} & \textbf{0.16}
                          \\
       & FPFH~\cite{5152473} + RANSAC~\cite{10.1145/358669.358692} & \textbf{1.52} & 4.40 & 2.65 & 4.12 & 1.18 & 3.97 & 4.10 & 8.48 & 1.03 & 3.07 & 3.04
                         \\
      & VF-NeRF + PC Init. &  1.61 & 6.30 & 2.65 & 1.96 & \textbf{0.15} & \textbf{0.19} & \textbf{0.34} & \textbf{0.26} & \textbf{0.65} & 1.45 & 1.93
      \\
       \bottomrule
     \end{tabular}
   }
 

 
   \label{table:full_objaverse_results}
  %  \vspace{-4mm}
\end{table*}

